Is Certifying $\ell_p$ Robustness Still Worthwhile?

Over the years, researchers have developed myriad attacks that exploit the ubiquity of adversarial examples, as well as defenses that aim to guard against the security vulnerabilities posed by such attacks. Of particular interest to this paper are defenses that provide provable guarantees against the class of $\ell_p$-bounded attacks. Certified defenses have made significant progress, taking robustness certification from toy models and datasets to large-scale problems like ImageNet classification. While this is undoubtedly an interesting academic problem, as the field has matured, its impact in practice remains unclear, thus we find it useful to revisit the motivation for continuing this line of research. There are three layers to this inquiry, which we address in this paper: (1) why do we care about robustness research? (2) why do we care about the $\ell_p$-bounded threat model? And (3) why do we care about certification as opposed to empirical defenses? In brief, we take the position that local robustness certification indeed confers practical value to the field of machine learning. We focus especially on the latter two questions from above. With respect to the first of the two, we argue that the $\ell_p$-bounded threat model acts as a minimal requirement for safe application of models in security-critical domains, while at the same time, evidence has mounted suggesting that local robustness may lead to downstream external benefits not immediately related to robustness. As for the second, we argue that (i) certification provides a resolution to the cat-and-mouse game of adversarial attacks; and furthermore, that (ii) perhaps contrary to popular belief, there may not exist a fundamental trade-off between accuracy, robustness, and certifiability, while moreover, certified training techniques constitute a particularly promising way for learning robust models.

==> 06_Discussion.tex <==
\section{\textbf{Discussion}}


% the attack persists in large models 

% the very basic defense does not work. 

% when things do not scale: 1. scale it through engineering 2. 

% direction of gradients.

% threat models change over time

% explore possible differences 

% measure the cost of attack, the defense (e.g. input filter). 

% geometrical charactierzation of LLMs.

\paragraph{\textbf{How to Effectively Improve Model Capacity for Robustness via Lipschitz-based Methods?}}
A series of studies find, either empirically or theoretically, that robust models require more model capability~\cite{schmidt2018adversarially, bubeck2021law, li2023clean, wang2023better, altstidl2023raising}. However, for certifiable models, especially those certified using Lipschitz-based methods, increasing the model capacity is not trivial. First of all, the certifiable classifiers should be Lipschitz, rendering attention-based architectures out-of-scope since they do not have a Lipschitz bound. Although some work~\cite{kim2021lipschitz, xucertifiably} proposes to modify the attention mechanism to make it Lipschitz, it gives rise to a second problem. The Lipschitz bound of the entire network is computed as the multiplication of every layer since we have $\text{Lip}(f\circ g)\leq \text{Lip}(f) \cdot \text{Lip}(g)$. The building blocks of the network should be designed so that the Lipschitz inequality can be tight, i.e., $\text{Lip}(f\circ g)$ should not be too much smaller than $\text{Lip}(f) \cdot \text{Lip}(g)$. Otherwise with a loose Lipschitz bound estimation, very few input samples can be certificated due to the large Lipschitz bound. Because of this problem, increasing network depth is less effective at increasing model capacity because the Lipschitz bounds may become less tight the more layers the model has (the more times this inequality is applied). This problem may also be the cause that Lipschitz based methods do not work very well for $\ell_1$ certification, since it is hard to obtain a tight Lipschitz bound estimation under $\ell_1$ norm. For $\ell_2$ norm, several special building blocks are designed to obtain a tight bound. Orthogonal weights~\cite{trockman21orthogonalizing, soc, prach2022almost, xu2022lot} are a promising solution since $\text{Lip}(f\circ g)= \text{Lip}(f) \cdot \text{Lip}(g)$ if $f$ and $g$ are orthogonal transformations. However, when applied to convolution, Fast Fourier Transform (FFT) and inverse FFT need to be applied, making these methods more difficult to scale to large-scale datasets in terms of both training and deployment. Hu et al.~\cite{hu2023scaling} proposed using a linear residual branch so that the Lipschitz estimate of the residual block can be compact, and show that this method can obtain non-trivial deterministic certification on ImageNet. However, linear residual blocks are less expressive than non-linear residual blocks. Effectively improving model capacity for certification models may further bridge the gap between VRA and standard accuracy.


% \paragraph{\textbf{Robustness in the Era of Generative Models}} 
% Firstly, local robustness needs new definition to fit into generative mdoels. The definition of local robustness requires a continuous input space to begin with, which is usually not the case for LLMs and the text prompt part of the multimodal models. Directly applying local robustness to text embeddings isn't a reasonable threat model because a perturbed embedding vector might not align with any token in the vocabulary. Conversely, introducing random tokens often has little impact on the semantic meaning of a prompt and these perturbations are far more noticeable than adversarial noise designed for images. Thus, the ability to introduce tokens into a prompt without altering its semantic content grants text adversaries greater flexibility than their vision counterparts, posing significant challenges in safeaguarding text models.

% Secondly, it is unclear

% As is argued in the earlier sections, the lack of robustness does not get resolved automatically when we managed to scale small models to the current largest ones, e.g. GPT-4. 


==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

